Multi Agent Pathfinding for Noise Restricted Hybrid Fuel Unmanned Aerial Vehicles

Multi Agent Path Finding (MAPF) seeks the optimal set of paths for multiple agents from respective start to goal locations such that no paths conflict. We address the MAPF problem for a fleet of hybrid-fuel unmanned aerial vehicles which are subject to location-dependent noise restrictions. We solve this problem by searching a constraint tree for which the subproblem at each node is a set of shortest path problems subject to the noise and fuel constraints and conflict zone avoidance. A labeling algorithm is presented to solve this subproblem, including the conflict zones which are treated as dynamic obstacles. We present the experimental results of the algorithms for various graph sizes and number of agents.

==> label_pseudocode.tex <==
\begin{algorithm}
        \SetKwInOut{Input}{input}
        \SetKwInOut{Output}{output}

        \Input{Time Cost Matrix: $T \in \R^{N \times N}$ \\ Edge Cost Matrix: $D \in \R^{N \times N}$ \\ Noise Restriction Matrix: $G \in \R^{N \times N}$ \\ Adjacency Matrix: $A \in \R^{N\times N}$\\ Energy Cost Matrix: $C \in \R^{N \times N}$ \\ Energy Transfer Matrix: $Z \in \R^{N \times N}$ \\ Initial Battery/Generator States: $B_0, Q_0$\\Starting node index: $S$\\ Final node index: $F$ \\MAPF constraints for agent:  $M$  \\}
        \Output{Minimum Cost Path and corresponding Generator Pattern for Single Agent}

\SetAlgoLined
 $H  \gets  \{ (d=0,t=0, B_0, Q_0) \}$  // Open Set \\
 % $H_i \gets \emptyset  \quad \forall i \in N, i \neq S$ \\
 $P \gets \emptyset  \quad \forall i \in N$  // Closed Set \\ 
  
 \While{$H \neq \emptyset $}{
 
 % FT = \textproc{Minimum}(H) \\
 FT = $\argmin_{f(\cdot)} H$ \\
 // Label FT: $(d_i^k, t_i^k, b_i^k, q_i^k)$ for node $i$ and associated path $X_k$, $Y_k$ \\
\For{$(j, t_j' = t_i^k + t_{ij}) \in $  successors$(i, t_i^k$)}{ \label{alg1:nbrnodes}
// Extend with generator on: \\
$X_a = [X_k, j]$, $Y_a = [Y_k, 1]$ \\
$(d_j^a, t_j^a, b_j^a, q_j^a) = (d_i^k  + D_{ij}, t_j', b_i^k - C_{ij} + Z_{ij}, q_i^k - Z_{ij})$ \label{alg1:labelgenon}\\
\uIf{Feasible($X_a$, $Y_a$) $and$ $(d_j^a, t_j^a) \notin M$ $and$ $j \not\in X_a$ and EFF($(d_j^a, t_j^a, b_j^a, q_j^a), H)$ }{ \label{alg1:feascheck1}
    $H \gets H \cup (d_j^a, t_j^a, b_j^a, q_j^a)$
    }
// Extend with generator off: \\
$X_b = [X_k, j]$  \\ 
$Y_b = [Y_k, 0]$ \\
$(D_j^b, t_j^b, b_j^b, q_j^b) = (D_i^k  + D_{ij}, t_j', b_i^k - C_{ij}, q_i^k)$ \label{alg1:labelgenoff} \\
\uIf{$Feasible$($X_b$, $Y_b$) $and$ $(d_j^b, t_j^b) \notin M$ and $j \not\in X_b$ and EFF($(D_j^b, t_j^b, b_j^b, q_j^b), H)$}{ \label{alg1:feascheck2}
    $H \gets \cup (D_j^b, t_j^b, b_j^b, q_j^b)$
    }
} %end for
% Remove $FT$ from untreated set $H$\\
% Add $FT$ to treated set $P$
$H \gets H \setminus FT$ \\
$P \gets P \cup FT$

} %end for 

\caption{Single Vehicle Labeling Algorithm} \label{algo:labeling}

\end{algorithm}
